A construction of deformations to general algebras

One of the questions investigated in deformation theory is to determine to which algebras can a given associative algebra be deformed. In this paper we investigate a different but related question, namely: for a given associative finite-dimensional C-algebra A, find algebras N which can be deformed to A. We develop a simple method which produces associative and flat deformations to investigate this question. As an application of this method we answer a question of Michael Wemyss about deformations of contraction algebras.

==> theory.tex <==


\section{Theory}

We have the following line of thinking:
\begin{enumerate}
    \item We let $A$ be a inite dimensional associative unital $\C$-algebra generated by $1, a $ and $b$ as an algebra. \dora{We might want $A$ to be a complex matrix algebra or semisimple.} \daveold{I want to fix a basis $B := \{e_i\}_{i = 1}^{\dim_{\C}(A)}$ in terms of $a,b$ here as it makes writing things precisely a bit easier.}
    \item Let 
    \[x:=ta, \quad y:=tb, \quad 1:= \mathbf{1},\]
    where $t$ is some fixed constant.
    \item Let $M$ be the algebra generated by $ta,tb$ and $1$, so a subring of $A[t]$. 
    \item  Note that $\C[x,y]$ is the free unital algebra generated by $x$ and $y$.
    \item Let $f:\C[x,y]\rightarrow M\subseteq A[t]$ be such that
    \[f:x\mapsto ta,\quad  f:y\mapsto tb, \quad f:1\mapsto 1.\]
    \dora{ $\C[x,y]$ is the free unital algebra on x and y, so it contains $1$ (and $\C$) and any words on x and y.} Note that this assignment determines $f$ on $\C[x,y]$ as $\C[x,y]$ is free.  

    Let's have a quick think about this. The algebra $M$ contains things like $\alpha, \beta t a, \gamma t b, \delta t^2 ab ...$ for $\alpha, \beta, \gamma, \delta \in \C$. \dora{Here I am assuming that $M$ inherits its multiplication from A[t]} \dave{Yes, this is one of the nice properties of this approach as we get associativty without having to engage with Hochschild Cohomology}. $M$ doesn't contain things like $\alpha t$ for $\alpha \in \C$. \dora{- Is this correct?} The algebra $\C[x,y]$ contains things like $\alpha, \beta x, \gamma y, \delta xyyx ...$ for $\alpha, \beta, \gamma, \delta \in \C$. In fact, $\C[x,y]$ is the free $\C$-module with basis being the free monoid on $x$ and $y$. Let's examine surjectivity and $\ker f$:
    \begin{itemize}
        \item Consider an arbitrary element of $M$, say $\alpha t^4abba$ where $\alpha\in \C$. Then $f:\alpha xyyx \mapsto \alpha t^4abba$. So it makes sense that $f$ is surjective. \dora{Task: give proof.}
        \item As the algebra $A$ could have some relations on it, the algebra $M$ could also have some relations. Note that the algebra $\C[x,y]$ has no relations on it as it is free. Hence $ker f$ could contain some non-zero elements.
    \end{itemize}

    \item Note that by the $1$st isomorphism theorem $M\cong \frac{\C[x,y]}{ker f}$ as $f$ is onto. 
    \item \doraa{Important point! This should be a ring where t commutes with everything, and not $\C[x,y,t]$} Extend the map $f$ to $f:\C[x,y,t]\rightarrow A[t]$ such that 
    \[f:x\mapsto at,\quad  f:y\mapsto bt, \quad f:t\mapsto t.\]
    We will denote $ker f$ by $I$. Let's examine this map.
    \begin{itemize}
        \item This map will not be injective as, for example, $txyt$ and $xytt$ both map to $t^4ab$.
        \item Consider some arbitrary element of $A[t]$, say $\alpha ababa t^7$ where $\alpha\in \C$. Then $f(\alpha t^2xyxyx) = \alpha ababa t^7$. It appears $f$ is onto. However I don't think that elements from $A$ are in the image of $f$. \dora{What is true?}.
        \item Consider $xyt\neq txy\in \C[x,y,t]$. Notice that $xyt-txy\in I=ker f$, so $I$ contains non-zero stuff (as expected). \dora{Find $I$.}
    \end{itemize}
    \item Let $i$ be the isomorphism $\C[x,y,t]/I\cong Im f$. Note that $Im f\subseteq A[t]$ is an algebra generated by $at, bt$ and $t$. \dave{cite image of algebra homomorphism is a subalgebra}
    \item Let $g: Im f \rightarrow A$ be such that 
    \[g:ta\mapsto a,\quad  g:tb\mapsto b, \quad g:t\mapsto 1.\]
    Note that $g$ is onto. \dora{We need to check g is well-defined. We would later like to calculate $\ker g$. Agata made a point that it might make sense to define $g$ on $A[t]$.}
    \item Let $h: \C[x,y,t]/I\rightarrow Im h$ be such that
    \[h:x\mapsto x,\quad  h:y\mapsto y, \quad h:t\mapsto 1.\]
    Then we have $\ker h = \{I, t-1\}$.
     \dora{Need to show $h$ is well defined. I am not sure if we had the map $h$ from $\C[x,y,t]$ instead of $\C[x,y,t]/I$. Not sure if it matters. 
     %Above $h$ is what we wrote in the meeting on the blackboard, but do we want
      %\[h:x\mapsto a,\quad  h:y\mapsto b, \quad h:t\mapsto 1,\]
      %if we want h to be onto. 
      Is this correct?}
      \item Let $\xi:\C[x,y,t]\rightarrow A$ be such that
      \[\xi:x\mapsto a,\quad  h:y\mapsto b, \quad h:t\mapsto 1.\]
      Then $\xi$ is onto. Note that $g\circ i\circ can (x)=\xi(x), g\circ i\circ can (y)=\xi(y)$ and $g\circ i\circ can (t)=\xi(t)$, so $g\circ i\circ can=\xi$.
\end{enumerate}
\bigskip

We have constructed the following diagram.


% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZARgBoAGAXVJADcBDAGwFcYkQAdDgYWQA9SAT1I5KIAL6l0mXPkIpypYtTpNW7LrwHDRAegCSEqSAzY8BImQBMKhizaIQ+gLYACABZHpZuZaW21Byc3ADMvExlzeWQrfxo7dUcAQQkVGCgAc3giUBCAJwhnJEUQHAgkMlV7dgBjekIaRnoAIxhGAAVI30c8rAz3HHD8wuKaMqQAFnjAjQ4+LCGCosQS8cQAZmnqxzDJXKWKsfKNrcSQBcaWts6fCx6+gcWRk9LjqaqzjJBL1o6uu5AvX6gz2IGGy0qa1iHyCnh+13+8kBDxBlHEQA
\begin{tikzcd}
                                               & {\C[x,y,t]} \arrow[ld, "can"'] \arrow[rd, "\xi"] \arrow[d, "f"] &   \\
{\C[x,y,t]/I} \arrow[r, "i"'] \arrow[rd, "h"'] & Im f \arrow[r, "g"']                                            & A \\
                                               & Im h                                                            &  
\end{tikzcd}

\dave{so we've thrown away $h$ entirely no?} \dora{We still keep h for the last proof below.}


















